Optimal learning rate schedules in high-dimensional non-convex optimization problems

Learning rate schedules are ubiquitously used to speed up and improve optimisation. Many different policies have been introduced on an empirical basis, and theoretical analyses have been developed for convex settings. However, in many realistic problems the loss-landscape is high-dimensional and non convex -- a case for which results are scarce. In this paper we present a first analytical study of the role of learning rate scheduling in this setting, focusing on Langevin optimization with a learning rate decaying as $\eta(t)=t^{-\beta}$. We begin by considering models where the loss is a Gaussian random function on the $N$-dimensional sphere ($N\rightarrow \infty$), featuring an extensive number of critical points. We find that to speed up optimization without getting stuck in saddles, one must choose a decay rate $\beta<1$, contrary to convex setups where $\beta=1$ is generally optimal. We then add to the problem a signal to be recovered. In this setting, the dynamics decompose into two phases: an \emph{exploration} phase where the dynamics navigates through rough parts of the landscape, followed by a \emph{convergence} phase where the signal is detected and the dynamics enter a convex basin. In this case, it is optimal to keep a large learning rate during the exploration phase to escape the non-convex region as quickly as possible, then use the convex criterion $\beta=1$ to converge rapidly to the solution. Finally, we demonstrate that our conclusions hold in a common regression task involving neural networks.

==> old_main_text.tex <==
\section{Introduction}

Learning rate schedules are recently used across all areas of modern machine learning in order to improve performance. However, in most cases, there is still a lack of beforehand understanding of which scheduler is most suited for a given problem. practitioners are faced with the following question: g e are posed with the fo

%%%%%
Given an optimization problem solvable with local algorithms such as SGD, a natural question is the following: what is the optimal learning rate schedule to find a solution as quickly as possible ? The practitioner is indeed confronted with a dilemma: if the model is in a basin, a faster decay of the learning rate will help converge faster to the minimum. But decaying the learning rate too fast can stop the dynamics before a convex basin is reached. Hence, a crucial tradeoff needs to be found.

This question has mostly been studied in the setup of convex problems, where the optimal schedule usually goes as $\lr(t)\sim 1/t$. However, deep neural networks are known to operate in non-convex landscapes: for example, due to the permutation invariance of any two nodes in a given layer, each global minimum in the loss landscape is replicated multiple times, with high loss barriers in the middle.

In such non-convex landscapes, one may ask: is the optimal learning schedule still $\lr(t)\sim 1/t$ ? 
To answer this question we consider various models, with various loss functions $\loss(x)$ and analyse the Langevin dynamics at temperature $T$ of the system :
\begin{align}
\label{eq:langevin}
    \begin{split}
        \frac{\dd \spin_i(t)}{\dd t} ) = - \lr(t)\left( \frac{\partial \loss(\spin)}{\partial x_i} + \spherical(t)\spin(t) - \xi(t) \right),
    \end{split}
\end{align}
where $\noise(t)$ is a Gaussian noise with $0$ mean and variance $\langle \noise(t) \noise(t^{\prime})\rangle = 2 T \delta(t-t^{\prime})$ and $\spherical(t)$ is a Lagrange multiplier imposing the spherical constrain $||\spin(t)||^2=N \quad \forall t$. We find both numerically and analytically, that a proper choice of learning rate schedule can benefit optimisation.

\paragraph{Related work}

Exploration of optimal learning rate scheduling has mostly been empirical. For a long time, stepwise decays of the learning rate have been used predominantly. But recently, an increasing body of research has turned to cosine annealing, which involves less hyperparameters to tune.

Before decaying the learning rate, an important question of study has been the use of learning rate warmup. 

\paragraph{Contributions}

In this paper, we present various frameworks with the general idea of showing that the higher the degree of non-convexity in the problem at hand, the slower the learning rate must be decayed.
We first study the classic Sherrington-Kirkpatrick spin glass model, showing that the optimal learning rate decay is $~1/t^\lrexponent$ with $\lrexponent=1/2$ instead of $1$ in the absence of a signal. 

However, in presence of a signal, the dynamics become more complex, and a crossover time emerges between two phases: an initial phase where the signal is not detected, where a high learning rate is favoured, followed by a second phase where the signal is detected and one must decay the learning rate as $1/t$ to converge optimally. These two phases are reminiscent of the warmup-then-anneal scheme which is commonly used in practice.

We then extend our findings to the spiked matrix-tensor model, showing that increasing the degree of non-convexity (exponential number of minima) pushes the optimal decay to $\lrexponent<1/2$, with $\lrexponent$ decreasing as we increase the non-convexity. 

Finally, we present numerical experiments in a teacher-student regression task, showing that overparametrizing the student also makes the problem more convex and favors faster decays of the learning rate.

\section{Warmup : a convex problem}
Consider the simplest model of a convex energy landscape: $\loss(\spin) = \frac{1}{2} \spin^2$.
We attempt to find a solution to the following Langevin equation: 
\begin{align}
    \dd\spin/\dd t = -\lr(t) (\dd\loss/\dd\spin + \noise(t)), \quad \langle \noise(t) \noise(t') \rangle = 2T \delta(t-t')
\end{align}

This equation is easy to solve, and yields
\begin{align}
    \spin(t) = \underbrace{\spin(t_0) e^{-\int_{t_{0}}^t \dd \tau \lr(\tau) }}_{\bar \spin(t)} + \underbrace{\int_{t_0}^t \dd t' e^{-\int_{t_0}^{t'} \dd t\tau \lr(\tau) }\lr(t') \noise(t')}_{\delta \spin(t)} 
\end{align}

Hence, 
\begin{align}
    \langle 2 \loss(t) \rangle &= \langle \bar \spin(t)^2 \rangle + \langle \delta \spin(t)^2 \rangle + 2 \underbrace{\langle \bar \spin(t) \delta \spin(t) \rangle}_{0}  \\ 
    &= \underbrace{\spin(t_0)^2 e^{-2\int_{t_0}^t \dd \tau \lr(\tau)}}_{\bar \loss(t)} + \underbrace{2T \int_{t_0}^t \dd t' \lr(t')^2 e^{-2\int_{t'}^{t} \dd \tau \lr(\tau)}}_{\delta \loss(t)} 
\end{align}

To converge to the solution as quickly as possible, one is faced with a dilemma: reducing the learning rate reduces the impact of the noise term, but also slows down the optimization. An ideal tradeoff is found when these two effects are comparable.

If we take $\lr(t)=\lr_0/t$, we obtain 
\begin{align}
    \bar \loss(t) &\propto e^{-2 \lr_0 \log(t)} \propto t^{- 2\lr_0} \\
    \delta \loss(t) &\propto \int_{t_0}^t \dd t' \frac{1}{t'^2} \left(\frac{t'}{t}\right)^{2\lr_0}  \propto t^{-1}
\end{align}
Hence, the loss decays to zero as $1/t$ if we take $\lr_0=1/2$.

Note that if we take a slower decay such as $\lr(t)\sim 1/\sqrt t$, $\bar \loss(t)$ converges to 0 exponentially fast, but $\delta \loss(t) \propto \lr(t)$  becomes limiting as it decays to zero slower. 

Conversely, if we take a faster decay such as $\lr(t) = \lr_0 \sim 1/t^2$, then the noise term decays rapidly but the dynamics will stop before the solution, as $\bar \loss(t) = e^{-2 \lr_0(1/t_0-1/t)}$ does not converge to zero when $t\to\infty$.

\section{A nonconvex setup: Sherrington-Kirkpatrick model}

As a hallmark of nonconvex optimization landscapes, we choose to study the simplest spin glass model, introduced by Sherrington and Kirkpatrick. In this model, a set of $N$ spins $\spin_i(t)$ try to to find the configuration minimizing their energy $\loss$, but are constrained to lie on a sphere:
\begin{align}
    \loss = -\frac{1}{2} \sum_{i\neq j} J_{ij} \spin_i \spin_j, \quad\quad\quad \Vert \spin \Vert^2 = \sum_i \spin_i^2 = N
\end{align}

The couplings $J_{ij}$ are sampled independently from $\mathcal N(0, 1/N)$. Hence, we know that in the $N\to\infty$ limit, the spectral density of $J$, defined as $\rho(\mu) = 1/N \sum_{i=1}^N \delta(\mu-\mu_i)$, converges to a semi-circle law:
\begin{align}
    \rho(\mu)=\frac{1}{2 \pi} \sqrt{4-\mu^{2}}, \quad \forall \mu \in[-2,2]
\end{align}

\paragraph{Dynamics}
Following~\cite{cugliandolo1995full}, we express the spin configurations in the eigenbasis of $J$, denoting $\spin_\mu = s\cdot J_\mu$ as the projection of $s$ onto the eigenvector $J_\mu$.
The corresponding Langevin equation can be written as follows:
\begin{align}
    \frac{\partial \spin_{\mu}(t)}{\partial t}= \lr(t) \left[ (\mu-\spherical(t)) \spin_{\mu}(t)+\noise_{\mu}(t)\right], \quad\quad\quad \langle \noise(t) \noise(t')\rangle = 2T \delta(t-t')
\end{align}
where $\spherical(t)$ is a Lagrange multiplier enforcing the spherical constraint.

Integrating this equation again gives two terms, one related to forgetting the initial condition, and one related to the noise:
\begin{align}
    \spin_{\mu}(t)= \underbrace{ \spin_{\mu}\left(0\right) e^{-\int_{0}^{t} d \tau \lr(\tau)(\mu-\spherical(\tau))}}_{\bar \spin_\mu(t)}+\underbrace{\int_{0}^{t} d t^{\prime \prime} e^{-\int_{t^{\prime \prime}}^{t} d \tau^{\prime}\lr(\tau^\prime) (\spherical(\tau^\prime)-\mu)}\lr(t^{\prime\prime})\noise_{\mu}\left(t^{\prime \prime}\right)}_{\delta \spin_\mu(t)}
\end{align}

\paragraph{Energy}
To obtain the energy as a function of time, one may notice a simple relation obtained by multiplying the langevin equation by $s$:
\begin{align}
    \langle \sum_\mu \spin_\mu \frac{\partial \spin_{\mu}(t)}{\partial t}\rangle &= \frac{\partial \Vert \spin \Vert^2}{\partial t} = 0\\
    &= \lr(t) \left[ \langle \sum_\mu \mu \spin_\mu (t)^2 \rangle - \spherical(t) \langle \sum_\mu \spin_\mu (t)^2 \rangle \right] + \lr(t) \langle \sum_\mu \delta \spin_\mu(t) \noise(t) \rangle\\
    &= \lr(t) \left[ - 2 \loss(t) - \spherical(t) \right] + \lr(t)^2 T
\end{align}

Hence,
\begin{align}
    \loss(t) = \frac{1}{2} \left(\lr(t) T - \spherical(t)\right)
\end{align}

Like before, we have one term related to the noise, which decays with $\lr(t)$, and another term linked to the optimization. Our objective is for these two terms to be on similar scales. To obtain the energy, we must find $\spherical(t)$ such that $\langle \int \dd \mu \rho (\mu) \spin_\mu(t) \rangle = 1 \ \forall t$. We will focus on the behavior of $\spherical(t)$ when $t\to\infty$.

\paragraph{Solving the self-consistent equation}
Now assume that $\lr(t)=\lr_0/t^\lrexponent$, with $\lrexponent<1$.

To avoid $\bar \spin_\mu$ from exploding, we need $\mu - \spherical(t)$ to be negative for all $\mu$ in the support of $\rho$, hence $\spherical(t)<2$. We also need $\spherical(t)\to_{t\to\infty} 2$, otherwise we will have $\spin_\mu(t)\to 0 \ \forall \mu$ which cannot satisfy the spherical constraint. Let's write $\spherical(t) = 2-f(t)$, with $f(t)\to_{t\to\infty}0$.

In the $\lrexponent=0$ setup, we know that $f(t) = c/t$~\cite{cugliandolo1995full}. Hence a natural ansatz is $f(t) = c/t^{1-\lrexponent}$. We must then ensure that 
\begin{align}
    1 &= \langle \int \dd \mu \rho (\mu) \spin_\mu(t)^2 \rangle \\
    &= t^{2c\lr_0} \int_{-2}^{2} \dd \mu \sqrt{4-\mu^2} e^{2\lr_0 (\mu-2) t^{1-\lrexponent}} \\
    %&= t^{2c\lr_0} \int_{-4}^{0} \dd \mu \sqrt{- 2\mu - \mu^2} e^{2\lr_0\mu t^{1-\lrexponent}} \\
    &= t^{2c\lr_0 - 3(1-\lrexponent)/2} \int_0^\infty \dd \epsilon \sqrt{2\epsilon} e^{-2\lr_0\epsilon}\\
    &\propto t^{2c\lr_0 - 3(1-\lrexponent)/2}
\end{align}
Hence we find $c=3(1-\lrexponent)/4\lr_0$, and we have:
\begin{align}
    \loss(t) - 1 = \underbrace{\frac{\lr_0 T}{2t^\lrexponent}}_{\delta \loss(t)} + \underbrace{\frac{3(1-\lrexponent)}{8 \lr_0 t^{1-\lrexponent}}}_{\bar \loss(t)} \sim  t^{-\min(\lrexponent, 1-\lrexponent)} \Rightarrow \lrexponent_\star = 1/2,
\end{align}
with $\loss_{GS}=-1$. Note that due to the finite temperature, the energy does no decay to the ground state $\loss(t)=-1$. Decreasing the learning rate has two adversarial effects: it reduces the noise term but increases the other term. Note that for $\lrexponent=0$ we recover the expression of~\cite{cugliandolo1995full}.

We validate this scaling by experiments at finite $N$, see Fig.~\ref{fig:exponents}. Note that the optimal learning rate schedule ensures that the second and third terms are equal. This imposes $\lrexponent=1/2$ and $\lr_0 = \sqrt{\frac{3}{16T}}$. In this case, the energy converges to zero at the rate $t^{-1/2}$, which was shown to be optimal for non-convex problems~\cite{agarwal2012information}.

\paragraph{Case $\lrexponent=1$}
For $\lrexponent=1$, we instead use the ansatz $\spherical(t) = 2-c/\log(t)$:
\begin{align}
    1 &= \int_{-2}^{2} \dd \mu \sqrt{4-\mu^2} e^{2\lr_0 (\mu-2) \log t} e^{2c\lr_0\log\log t} \\
    &= (\log t)^{2c\lr_0 - 3/2} \int_0^\infty \dd \epsilon \sqrt{2\epsilon} e^{-2\lr_0\epsilon} \\
    &\propto  (\log t)^{2 c\lr_0 -3/2}
\end{align}

Hence the energy decays does not decay algebraically anymore, but logarithmically:
\begin{align}
    \loss(t) - \loss_{GS} = \frac{\lr_0 T}{2t} + \frac{3}{8 \lr_0 \log t} \sim  (\log t)^{-1}
\end{align}

\paragraph{Dependency on the spectrum of $J$}
One may naturally ask whether our conclusions are affected by changing the spectrum of the coupling matrix $J$. Notice that the key to solving the self-consistent equation is the behavior of the spectrum near its right edge. For the semi-circle law considered here, the right edge of the spectrum behaves as a square root. This law applies to a rather wide range of random matrix ensembles. Besides, many other common spectral densities, such as the Marcenko-Pastur law, also exhibit a same square root behavior on their right edge. Hence we expect our results to hold for a wide range of random matrix ensembles.

% Our computation is valid in the $N\to\infty$ limit. However, finite-size effects turn out to be important in this problem. As shown in~\cite{fyodorov2015large}, there is a cross-over time $\tjump\sim N^{2/3}$ above which the system enters a new regime. In this regime, the system becomes aligned with the strongest eigenmode of $J$ and the landscape becomes almost quadratic. In this regime, using a more aggressive decay of the learning rate becomes helpful, as shown in Fig.~\ref{fig:crossover}. Instead of observing a logarithmic decay of the energy as observed at early times, we observe a $1/t$ decay. Hence, due to the finite size effects, the optimal learning rate schedule consists in using $1/\sqrt t$ up to the crossover time, then using $1/t$ at late times. 

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{figs/energy_psm_spike_0.pdf}
%     \caption{Without spike}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{figs/energy_psm_spike_2.pdf}
%     \caption{With spike $c=2$}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{figs/energy_psm_spike_10.pdf}
%     \caption{With spike $c=10$}
%     \end{subfigure}
%     \caption{How different learning rate schedules affect the energy as function of time. We set $N=1000$, $T=2$, $\lr_0=0.5$.}
%     \label{fig:crossover}
% \end{figure}

\section{When signal induces convexity: the two phases of learning}
\label{sec:crossover}

We now move to the setup where there is a "signal" in the problem, which must be retrieved. To mimick this, one could keep the SK model, but add a rank-one matrix to the couplings $J$:
\begin{align}
    \tilde J_{ij} = J_{ij} + \lambda \signal_i \signal_j, \quad\quad\quad \signal_i\sim\mathcal N(0,1)
\end{align}

In this case, an eigenvalue pops out of the bulk when $\lambda \geq 2$. The spectrum then takes the following form:
\begin{align}
    \rho(\mu) = \frac{N-1}{N} \rho_{sc}(\mu) + \frac{1}{N} \delta(\mu-\lambda)
\end{align}

In the following, we define $\lambda-2 \equiv \Delta$.

\paragraph{Emergence of a crossover time}
Again we choose $\lr(t)=\lr_0/t^\lrexponent$ and set $\spherical(t) = \lambda - f(t)$:
\begin{align}
    1 &= \langle \int \dd \mu \rho (\mu) \spin_\mu(t)^2 \rangle \\
    &= \frac{N-1}{N}\int_{-2}^{2} \dd \mu \rho_{sc}(\mu) e^{2\int_{t_0}^t \dd \tau \lr(\tau) (\mu-\lambda) } e^{2\int_{t_0}^t \dd \tau \lr(\tau) f(t)} + \frac{1}{N} e^{2\int_{t_0}^t \dd \tau \lr(\tau) f(t)}\\
    &= e^{2\int_{t_0}^t\dd \tau \lr(\tau) f(\tau)} \left( \underbrace{e^{-2\lr(t)(\lambda-2) t}\int_{-2}^{2} \dd\mu \rho_{sc}(\mu) e^{2\lr(t)(\mu-2) t}}_{A(t)} + \frac{1}{N}\right)
    \label{eq:competition}
\end{align}

The expression above involves two terms. The first is of order one but decays over time:
\begin{align}
    A(t)\sim
    t^{-3(1-\lrexponent)/2}e^{-2\lr_0\Delta t^{1-\lrexponent}}
    %\sim e^{-2\lr_0\Delta t^{1-\lrexponent}} 
\end{align}
Hence there is a crossover time at which it becomes smaller than the second term, given by:
\begin{align}
    A(t)\sim1 \Rightarrow \tjump = 
    \left( \frac{\log N}{2\lr_0 \Delta }\right)^{\frac{1}{1-\lrexponent}}
\end{align}

Before $\tjump$, the signal is not detected and we have as before $\spherical(t) = 2-c/ t^{1-\lrexponent}$. 

After $\tjump$, we have $A(t)\ll 1/N$, hence we can rewrite Eq.~\ref{eq:competition} as:
\begin{align}
    \log N &= 2 \int_{t_0}^t\dd \tau f(\tau) t^{-\lrexponent} + \log\left( 1 + N A(t)\right)\sim 2 \int_{t_0}^t\dd \tau f(\tau) t^{-\lrexponent} + N A(t)
\end{align}

Taking the derivative of this equation with respect to $t$, we find the following asymptotics for late times:
\begin{align}
    f(t) \sim \frac{-A'(t)t^\lrexponent}{2} \sim t^{-5(1-\lrexponent)/2} e^{-2\lr_0\Delta t^{1-\lrexponent}}
\end{align}

Hence,
\begin{align}
    \loss(t)-\loss_{GS} = \frac{\lr_0 T}{2t^{\lrexponent}} + \frac{1}{2} f(t)
\end{align}

with $\loss_{GS}=\lambda$. Since the second is exponentially decaying, it is tempting to write $\loss(t)-\loss_{GS} \sim t^{-\lrexponent}$, which would lead $\lrexponent=1$ to be optimal as in the convex setup. Interestingly however, $\lrexponent=1$ would cause $f(t)$ to remain constant, bottlenecking the dynamics. Hence, the problem is not purely convex: we need to choose $\lrexponent=1-\epsilon$ with $\epsilon\ll 1$, and also must beware that the decay of $f(t)$ will be slow as long as $t<(2\lr_0\Delta)^{-1/\epsilon}$, which can be large in practical cases where $2\lr_0\Delta\ll 1$.

\paragraph{Optimal learning rate schedule}

Let us now summarize the results obtained above.

To speed up the initial phase where the signal hasn't yet aligned with the signal, we need to reduce $\tjump$. To do so, one should use a large learning rate $\lr_0$ without any decay ($\lrexponent=0$). Passed this crossover, we enter a quasi-convex phase (the problem becomes essentially quadratic), and the optimal exponent becomes $\lrexponent=1-\epsilon$, with $\epsilon\ll 1$, in contrast with the vanilla SK model where $\lrexponent=1/2$ was optimal. 

Hence, the best schedule is to keep the learning rate constant up to $\tjump$, then decay with a strong exponent. This is confirmed by the experiments of Fig.~\ref{fig:crossover}.


\paragraph{Finite-size effects in the vanilla SK model}

In fact, even in the scenario without signal ($\lambda=0$), finite-size effects cause the $1/\sqrt t$ schedule to be suboptimal. Indeed, there is a finite gap between the largest and second largest eigenvalue at finite $N$, which is known to scale as $\Delta \sim N^{-2/3}$~\cite{perret2015density}. This creates a crossover time beyond which the problem becomes convex, given by:
\begin{align}
    \tjump \sim \left( \frac{N^{2/3}\log N}{2\lr_0 }\right)^{\frac{1}{1-\lrexponent}}
\end{align}

As a consequence, instead of using $\lr(t)\sim1/\sqrt t$ as prescribed for $N\to\infty$, for finite size systems the best schedule is to first use a large constant learning rate up to $\tjump\sim N^{2/3}$ at which point the problem becomes convex, then decay with a strong exponent. 

\begin{figure}
    \centering
    \includegraphics[width=.4\linewidth]{figs/energy_psm_exponents.pdf}
    \caption{\textbf{At infinite size, the optimal learning rate schedule to balance noise and forgetting of initial conditions is inverse square root.} In dashed lines, we predicted the theoretical convergence rate, given by $\min(\lrexponent, 1-\lrexponent)$. Note that since we the simulations are performed at finite size, the scaling will only hold up to the crossover time (see Sec.~\ref{sec:crossover}), which happens to be larger than the simulation time here. We set $N=1000$, $T=1$, $\lr_0=0.1$.}
    \label{fig:exponents}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/energy_psm_spike_2.pdf}
    \caption{\textbf{At finite size, or in presence of a signal, it is optimal to keep a constant learning rate until the crossover, then decay with a strong exponent.} We display the energy (left) and magnetisation (middle, i.e. overlap with the strongest mode of $J$) at constant learning rate $\lr_0=0.1$. Then, we select various points along the optimization path, and start new runs from these points but with a learning rate decaying as $\lr(t)=\lr_0/t^\lrexponent$, as shown in the the rightmost panel (colored lines, from blue to green). The dashed red line marks the theoretical crossover time $\tjump=\frac{\log N}{2 \lr_0 \Delta}$: we see that it matches with the moment when the loss saturates at constant learning rate. Before the crossover, decaying the learning rate is detrimental. After the crossover, it allows the model to converge to the ground state as $t^{-\lrexponent}$ (dashed grey line).
    We set $N=1000, T=0.1, \lr_0=0.1, \lrexponent=0.8, \Delta=0.5$.}
    \label{fig:crossover}
\end{figure}


\section{The p-spin model}
We now turn to the analysis of the p-spin model, in both its version with and without a ground truth signal $\signal$. 
It is a natural candidate for our analysis as its loss landscape is extremely complex and non convex and its dynamics are exactly solvable.


\subsection{Without signal}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{figs/pspin/NoSignal_T0.pdf}   
        \caption{Zero temperature}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{figs/pspin/NoSignal_T1.pdf}    
        \caption{Temperature $T=1$}
    \end{subfigure}
    \caption{\textbf{Top:} at zero temperature the energy of the p-spin model decays to the threshold energy as a power-law in time, $\loss-\loss_{\textbf{th}}\propto \lr_0 t^{-\delta}$. \textbf{Bottom}: At finite temperature the decay towards the power-law . \textbf{From left to right}: 3- spin model, 4-spin model, 6-spin model, and the corresponding decay rates as a function of $\lrexponent$. The exponent of the power law is $\delta = \frac{2}{3}(1-\lrexponent)$ as predicted by the scaling law \ref{eq:scaling_pspin}. $N=3000$, $T=0$, $\lr_0=0.5$.}
    \label{fig:pspin_noSignal}
\end{figure}

Consider first the unplanted, i.e. with no signal, version of the p-spin model having loss function:
\begin{equation}
    \label{eq:Hpdspin}
    \loss(t) = -\sqrt{ \frac{p!}{2 N^{p-1}}} \sum_{i_1<...<i_p} J_{i_1...i_p} \spin_{i_1}... \spin_{i_p}
\end{equation}
where the components of $J_{i_1...i_{p}}$ are drawn i.i.d. from a standard normal distribution. This model features \emph{extremely} slow relaxation dynamics and was first studied as a good playground to understand real spin glasses. 
\emph{discuss aging a bit and the phenomenology and complex landscape}

In the infinite system size limit $N\to\infty$, the dynamics of this model given by Eq.~\ref{eq:langevin} are described by a closed set of PDEs for the key macroscopic quantities. These are the self-alignment of the spins at different times $C(t,t')~=~\lim_{N\to\infty}\nicefrac{1}{N}\EE_{\noise}\sum_{i=1}^N \spin_i(t)\spin_i(t')$ and the response of the system to a perturbation in the loss function at previous time $R(t,t')~=~\lim_{N\to\infty}\nicefrac{1}{N}\EE_{\noise}\sum_{i=1}^N\delta \spin_i(t)/\delta \xi_i(t')$. 
In the $N\to\infty$ limit, $C$ and $R$ converge to non fluctuating limit i.e. they concentrate with respect to the randomness in the coupling $J$ and of the thermal noise in the dynamics $\noise$. Their dynamics is described by a closed set of equations which we derive following the methods of \cite{castellani2005spin}. More details is given in  App.~\ref{app:derivationNoSignal}.
\begin{align}
\label{eq:dynamical_equations_no_signal}
\frac{\partial R\left(t_{1}, t_{2}\right)}{\partial t_{1}}=&-z\left(t_{1}\right)\lr(t_1) R\left(t_{1}, t_{2}\right)+ \lr(t_1)\delta\left(t_{1}, t_{2}\right)\\
& +\frac{p(p-1)}{2}  \lr(t_1)\int_{t_{2}}^{t_{1}} d t^{\prime \prime} \lr(t^{\prime\prime}) R\left(t_{1}, t^{\prime \prime}\right) C^{p-2}\left(t_{1}, t^{\prime \prime}\right) R\left(t^{\prime \prime}, t_{2}\right)
\\
\frac{\partial C\left(t_{1}, t_{2}\right)}{\partial t_{1}}=& -\lr(t_1)z\left(t_{1}\right) C\left(t_{1}, t_{2}\right)+ 2T\lr(t_1)^2 R(t_1, t_2)\\
&+\frac{p(p-1)}{2} \lr(t_1) \int_{-\infty}^{t_{1}} d t^{\prime \prime} \lr(t^{\prime\prime})R\left(t_{1}, t^{\prime \prime}\right) C^{p-2}\left(t_{1}, t^{\prime \prime}\right) C\left(t^{\prime \prime}, t_{2}\right) \\
&+ \frac{p}{2}\lr(t_1) \int dt^{\prime\prime} \lr(t^{\prime\prime}) R(t^{\prime\prime}, t_2) C^{p-1}(t^{\prime\prime}, t_1)\\
\spherical(t) =& T\lr(t) + \frac{p^2}{2}\int dt_2 \lr(t_2) R(t_2, t_1) C^{p-1}(t_2, t_1).
\end{align}
The initial conditions are $R(t,t^{\prime})=0\quad\forall t^{\prime}>t$, $\lim_{t^{\prime}\to t^-}R(t,t^{\prime})=1$ and $C(t,t)=1\quad \forall t$ which allows to find the last equation for the Langrange multiplier enforcing the spherical constrain. 
To obtain the energy, we use, as in the $p=2$ case, the spherical constrain combined with Ito's lemma:
\begin{align}
\label{eq:loss_pspin_no}
\begin{split}
\frac{\partial ||\spin||^2}{\partial t} &= 0\\
\Rightarrow  
   \loss(t)& = \frac{-1}{p}\left(  \spherical(t) - T \lr(t) \right )
\end{split}
\end{align}

The loss is the sum of two competing terms: one related with optimisation $\spherical(t)$ and the other with fluctuations in the optimisation $T \lr(t)$. Since the temperature is fixed, by choosing a learning rate $\lr(t)=\nicefrac{\lr_0}{t^{\lrexponent}}$, the later decays as $t^{-\lrexponent}$. 

The decay of the former is more complex due to the high complexity of the landscape. It can be shown \cite{cugliandolo1995full} that system never reaches the ground state and the dynamics remain trapped in metastable minima at a threshold energy:
\begin{equation}
   \loss_\th= \sqrt{\frac{ 2 (p-1) }{ p}}.
   \label{eq:energy_threshold}
\end{equation}

At constant learning rate, the relaxation of the dynamics towards the threshold states is characterised by a power-law decay of the loss with exponent $\delta$. In \cite{thalmann2001geometrical}, the authors establish that the $T=0$ exponent $\delta=\nicefrac{2}{3}$ i.e. $\spherical_\th - \spherical(t)\propto t^{-\delta}$.
We consider how this decay changes when a non constant learning rate $\lr(t)=\lr_0 t^{-\lrexponent}$ is chosen. Consider the time re-scaling:
\begin{align}
\begin{split}
    \dd\tilde{t} =\lr(t)\dd\tilde{t}
    \Rightarrow \tilde{t} = \begin{cases} 
                                \frac{t^{1-\lrexponent}}{1-\lrexponent}\qquad \text{if }\lrexponent<1\\
                                \log(t)\qquad \text{if }\lrexponent=1
                            \end{cases} .
    \end{split}
\end{align}
Using the first equation of Eqs.~\ref{eq:dynamical_equations_no_signal} with $T=0$, we obtain:
\begin{align}
\begin{split}
    \spherical(\tilde{t}_1) =& \frac{p^2}{2} \int_0^{\tilde{t}_1} \dd\tilde{t}_2 R(\tilde{t}_2, \tilde{t}_1) C^{p-1}(\tilde{t}_2, \tilde{t}_1).
    \end{split}
\end{align}
The integral above is exactly the one the authors of \cite{thalmann2001geometrical} obtain and scales as:
\begin{align}
   \spherical_\th - \spherical(t)\propto \tilde{t}^{-\delta} \propto\begin{cases} 
                                                                 t^{-\delta(1-\lrexponent)}\qquad \text{if }\lrexponent<1\\
                                                                 \log(t)^{-\delta}\qquad \text{if }\lrexponent=1
                                                            \end{cases}.
\end{align}
In Fig.~\ref{fig:pspin_noSignal}, we integrate Eqs.~\ref{eq:dynamical_equations_no_signal} for $p=3, 4, 6$ and check that, at $T=0$, the loss decays with an exponent $\delta (1-\lrexponent)= \nicefrac{2}{3}(1-\lrexponent)$ for $\lrexponent<1$.
Thus, the loss in Eq.~\ref{eq:loss_pspin_no} decays as a power law with exponent given by the the minimum between $\lrexponent$ and $\delta (1-\lrexponent)$. The value of $\lrexponent$ giving fastest optimisation is thus:
\begin{align}
    \begin{split}
        \label{eq:betaopt_pspin}
        \lrexponent_\opt = \delta (1-\lrexponent_\opt)\\
        \Rightarrow  \lrexponent_\opt = \frac{\delta}{\delta+1} = \frac{2}{5}
    \end{split}
\end{align}
In Fig.~\ref{fig:pspin_noSignal}, we plot how the decay of $\loss$ towards $\loss_\th$, for $T=0$ and three values of $p$ and various $\lrexponent$. On the right hand most figure, we show the exponent of the curves as a function of $\lrexponent$. 
For $\lrexponent<\lrexponent_\opt$ the decay of the loss is limited by the noise term: the loss decreases as $t^{-\lrexponent}$. If $\lrexponent>\lrexponent_\opt$ the $z(t)$ term slows down the dynamics and the loss decays as $t^{-\delta(1-\lrexponent)}$. At $\lrexponent_\opt=0.4$, there is a p-independent sweet-spot where optimisation is fastest.

An alternative argument to find the $0$ temperature exponent, is to re-parametrise the time directly in the Langevin equation:
\begin{align}
    \begin{split}
        \frac{\partial \spin}{\partial t} = -\lr(t)\partial_{\spin} \loss + \noise(t) \qquad \langle\noise(t)\noise(t^\prime)\rangle = 2 T \delta(t-t').
    \end{split}
\end{align}

Define $\dd\tilde{t}=\lr(t)\dd t$. Then we have:
\begin{align}
\begin{split}
    \delta(\tilde{t} ) \dd \tilde{t}  =\delta(t) \dd t \Rightarrow \delta(t) &= \delta(\tilde{t} ) \lr  \left(\left((\lrexponent-1) \tilde{t}\right)^{\frac{1}{1-\lrexponent}}\right) \\
    &= \delta(\tilde{t} )(1-\lrexponent)^{\nicefrac{1}{1-\lrexponent}}t^{\nicefrac{-\lrexponent}{1-\lrexponent}}   
\end{split}
\end{align}
The Langevin equations of motion becomes:
\begin{align}
    \begin{split}
        \frac{\partial \spin}{\partial t} = -\partial_{\spin} \loss + \noise(t) \qquad \langle\noise(t)\noise(t^\prime)\rangle = 2 T (1-\lrexponent)^{\nicefrac{1}{1-\lrexponent}} t^{\nicefrac{-\lrexponent}{1-\lrexponent}}    \delta(t-t').
    \end{split}
\end{align}
This equation reveals that the process optimised with a varying learning rate is equivalent to a process with an effective temperature:
\begin{equation}
    \tilde{T} =  (1-\lrexponent)^{\frac{1}{1-\lrexponent}}\frac{T}{ t^{\nicefrac{\lrexponent}{1-\lrexponent}} }.
\end{equation}
The loss can therefore be written:
\begin{equation}
    \loss(t; \tilde{T})= \loss(t; T=0) + \loss_\th(\tilde{T})
\end{equation}
where we assumed that, at all times, the temperature dependent contribution to the energy has time to equilibrate in the threshold states.

To find $\loss_\th(\tilde{T})$, we assume that, since we are looking at long times, we have $\tilde{T}\ll 1$. We can consider the energy by performing an expansion around the $\tilde T=0$ minimum i.e. considering that the motion is oscillatory around the minimum. At $T=0$, the threshold overlap is given by $q_{\th}=1$. At $T\ll 1$, we thus write $q = 1- \chi T$. Performing a similar matching argument as the one of \cite{mannelli2020marvels}, we find that the close to the threshold, the energy is given by:
\begin{align}
\begin{split}
\label{eq:Lossth1}
    \loss_\th(T) &= -\frac{1}{p}\left[\sqrt{\frac{p(p-1)}{2}q^{p-2}} + \frac{p}{2 T}\left(1 - q^{p-1}\right)\right]
    \end{split}
\end{align}
In addition, we can expand the threshold overlap solution around $T=0$:
\begin{align}
    \begin{split}
        q_\th^{p-2} (1-q_\th)^2 &= T^{2}\frac{2}{p(p-1)}\\
        \Rightarrow \chi = \sqrt{\frac{2}{p (p-1)}}
    \end{split}
\end{align}
Replacing this solution in Eq.~\ref{eq:Lossth1}, we find:
\begin{align}
    \begin{split}
        \loss_\th(T) &= \underbrace{ - \sqrt{\frac{2(p-1)}{p}}}_{\loss_\th(T=0)} + \underbrace{\frac{(p-2)}{p}T}_{\propto T}
    \end{split}
\end{align}

We see that $\loss_\th(T)$ is composed of a constant term, which is the same as the threshold loss defined in Eq.~\ref{eq:energy_threshold} and a term scaling linearly with $T$. Thus:
\begin{align}
    \begin{split}
        \loss_\th(\tilde T) - \loss_\th \propto \tilde T \propto t^{- \nicefrac{\lrexponent}{1-\lrexponent}}.
    \end{split}
\end{align}
We find again the two competing term in the speed of optimisation. 
On the one hand, the noiseless term, which is the same as the zero temperature loss, decays as $\loss(t; T=0)\propto t^{-\delta}$. On the other hand, the temperature dependent term, which blocks the dynamics at energy $\loss_\th(\tilde T)$, which decays as $t^{-\nicefrac{\lrexponent}{1-\lrexponent}}$. The energy decays as $t^{-\mathrm{min}\left(\delta, \frac{\lrexponent}{1-\lrexponent}\right)}$. Equaling the two exponents gives the optimal value of $\lrexponent_\opt=\frac{2}{5}$.

\subsection{With signal}

\begin{figure}
    \centering
        \includegraphics[width=\linewidth]{figs/pspin/pspin_Signal.pdf}   
        \caption{\textbf{The optimal schedule is to use a constant learning rate until $\tjump$ and then to decay it with $\lrexponent=1$} \emph{(Left)} By fixing $\lrexponent$ from start, a randomly initialised system will remain stuck at \emph{threshold} states of $0$ magnetisation until $\tjump$ which is minimal for $\lrexponent=0$. Higher $\lrexponent$, allow to reach lower energy solution of higher magnetisation at finite times. \emph{(Right)} The optimal schedule is to keep $\lr$ constant until $\tjump$ and then setting $\lrexponent=0$. By doing so, we get the best of both worlds: the first phase minimises $\tjump$ while the second allows to reach more informative solutions. \emph{(Inset)} $m-m_\gs$ shows that choosing higher $\lrexponent$ after $\tjump$ allows to reach more informative minima. }
    \label{fig:pspin_Signal}
\end{figure}
As we did for the SK model, we consider the planted p-spin spherical model, a variant of the p-spin model with an addional signal term. Planting permits the introduction of a ground truth signal. In the neural-network language, this is often referred to as the \emph{teacher-student} scenario: the teacher has knowledge of the ground truth and uses it to generate data. The student uses the data to recover the signal. The spiked tensor model has been extensively studied in \cite{mannelli2019afraid, mannelli2020marvels, mannelli2019passed}. 
The observations are a matrix $Y_{ij}$ and a third order tensor $T_{ijk}$ generated from a ground truth $\signal$. The hardness of the problem is controlled via the intrinsic Gaussian noise of $Y$ and $T$ with variance $\Delta_2$, respectively $\Delta_p$. Note that the matrix term has to be included in order for the signal to be recovered at finite $\Delta_p$. The loss function is thus given by:
\begin{equation}
    \label{eq:Hpdspin_signal}
\loss(\spin) =\loss_{2}+\loss_{p}=-\frac{1}{\Delta_{2} \sqrt{N}} \sum_{i<j} Y_{i j} \spin_{i} \spin_{j} -\frac{\sqrt{(p-1) !}}{\Delta_{p} N^{(p-1) / 2}} \sum_{i_{1}<\cdots<i_{p}} T_{i_{1} \ldots i_{p}} \spin_{i_{1}} \ldots \spin_{i_{p}}
\end{equation}
with 
\begin{align}
Y_{i j} &=\frac{1}{\sqrt{N}} \spin_{i}^{*} \spin_{j}^{*}+\sqrt{\Delta_2}\noise_{i j} \quad \forall i<j \\
T_{i_{1} \ldots i_{p}} &=\frac{\sqrt{(p-1) !}}{N^{(p-1) / 2}} \spin_{i_{1}}^{*} \ldots \spin_{i_{p}}^{*}+\sqrt{\Delta_p}\noise_{i_{1} \ldots i_{p}} \quad \forall i_{1}<\ldots<i_{p}
\end{align}
with both $\noise_{i j}$ and $\noise_{i_{1} \ldots i_{p}}$ sampled i.i.d. from $\mathcal{N}(0,1)$.
Considering once more the Langevin dynamics Eq.~\ref{eq:langevin}, in the limit of infinite size, one can obtain a closed set of PDEs describing the dynamical evolution of the relevant variables in the system i.e. the overlap of the system with the ground truth $m(t)~=~\lim_{N\to\infty}\nicefrac{1}{N}\EE_{\noise}\sum_{i=1}^N \signal_i \spin_i(t)$, which describes how good the estimator $\spin$ is, the self-alignement of the estimator at different times $C(t,t')~=~\lim_{N\to\infty}\nicefrac{1}{N}\EE_{\noise}\sum_{i=1}^N \spin_i(t)\spin_i(t')$ and the response of the system to a perturbation in the loss function at previous time $R(t,t')~=~\lim_{N\to\infty}\nicefrac{1}{N}\EE_{\noise}\sum_{i=1}^N\delta \spin_i(t)/\delta \xi_i(t')$.
\begin{align}
    \begin{split}
&\frac{\partial}{\partial t} C\left(t, t^{\prime}\right)=-\spherical(t)\lr(t) C\left(t, t^{\prime}\right)+\lr(t)Q^{\prime}(m(t)) m\left(t^{\prime}\right)+\lr(t)\int_{0}^{t}\lr(t^\prime) R\left(t, t^{\prime \prime}\right) Q^{\prime \prime}\left(C\left(t, t^{\prime \prime}\right)\right) C\left(t^{\prime}, t^{\prime \prime}\right) d t^{\prime \prime} \\
&\quad+\lr(t)\int_{0}^{t^{\prime}}\lr(t^\prime) R\left(t^{\prime}, t^{\prime \prime}\right) Q^{\prime}\left(C\left(t, t^{\prime \prime}\right)\right) d t^{\prime \prime}+ 2T\lr(t)^2 R(t,t^\prime) \\
&\frac{\partial}{\partial t} R\left(t, t^{\prime}\right)=-\spherical(t)\lr(t) R\left(t, t^{\prime}\right)+\lr(t)\int_{t^{\prime}}^{t}\lr(t^\prime) R\left(t, t^{\prime \prime}\right) Q^{\prime \prime}\left(C\left(t, t^{\prime \prime}\right)\right) R\left(t^{\prime \prime}, t^{\prime}\right) d t^{\prime \prime} + \delta(t-t^\prime) \lr(t) \\
&\frac{d}{d t} m(t)=-\lr(t)\spherical(t) m(t)+\lr(t)Q^{\prime}(m(t))+\lr(t)\int_{0}^{t} \lr(t^\prime)R\left(t, t^{\prime \prime}\right) m\left(t^{\prime \prime}\right) Q^{\prime \prime}\left(C\left(t, t^{\prime \prime}\right)\right) d t^{\prime \prime} \\
&\spherical(t)=\lr(t)T+Q^{\prime}(m(t)) m(t)+\int_{0}^{t}\lr(t^\prime) R\left(t, t^{\prime \prime}\right)\left[Q^{\prime}\left(C\left(t, t^{\prime \prime}\right)\right)+Q^{\prime \prime}\left(C\left(t, t^{\prime \prime}\right)\right) C\left(t, t^{\prime \prime}\right)\right] d t^{\prime \prime}
    \end{split}
\end{align}
where we defined $Q(\spin)=Q_p(\spin)+Q_2(\spin)=\frac{\spin^{p}}{p \Delta_{p}}+\frac{\spin^{2}}{2 \Delta_{2}}$. The initial conditions are $R(t,t^{\prime})=0\quad\forall t^{\prime}>t$, $\lim_{t^{\prime}\to t^-}R(t,t^{\prime})=1$ and $C(t,t)=1\quad \forall t$ which allows to find the last equation for the Langrange multiplier enforcing the spherical constrain. 
In addition, using Ito's Lemma as before, we find that $z(t)$ is related to the loss via:
\begin{equation}
   \spherical(t) =\lr(t)T - 2 \loss_2 - p \loss_p.
\end{equation}

The phenomenology of the model varies depending on the values of $\Delta_p$ and $\Delta_2$ \cite{mannelli2019afraid}. Here, we focus on a regime where $\Delta_p$ is small enough and $\Delta_2$ is large enough and the problem is \emph{Langevin easy} i.e. starting from very small initial overlap with the ground truth, the Langevin dynamics will recover the signal.
The boundaries of this region is given by $\Delta_2^*$ as:
\begin{equation*}
    \Delta_2^* =\sqrt{ \frac{\Delta_p }{ (p-1)  (1-\Delta_2^{*})^{p-3} ) }}
\end{equation*}
If $\Delta_2<\Delta_2^*$, the Langevin dynamics initialised at random fails to recover the signal and remains at $m(t)=0$ magnetisation. 

The dynamics of the easy phase have been well understood at constant learning rate $\lr_0=1$ in \cite{mannelli2019passed, mannelli2019afraid, mannelli2020marvels}. The authors show that the system remains trapped in \emph{threshold states} until a time $\tjump$ which increases the closer $\Delta_2$ is to $\Delta^*_2$ (i.e. the smaller $\Delta_2-\Delta^*_2$ is). At $\tjump$, the magnetisation increases exponentially fast and converges to $m_\gs$. 
Fig.~\ref{fig:pspin_Signal} shows how changing the learning rate with time can improve optimisation similar to what we observed for the SK model. On the left, we fix from start a learning rate $\lr(t)=\lr_0 t^{-\lrexponent}$ for various $\lrexponent$. We see that a constant learning rate (i.e. $\lrexponent=0$) allows to minimise $\tjump$, the time the system takes to identify the signal. However, increasing $\lrexponent$ enables the system to reach higher magnetisation i.e. to have a better estimate of the ground truth. We thus conclude that the best schedule, used in Fig.~\ref{fig:pspin_Signal} (right) s to keep $\lrexponent=0$ until $\tjump$ and to then decrease the learning rate with $\lrexponent = 1$ i.e. $\eta(\tau = t-\tjump)=\nicefrac{1}{\tau}$ in order to reach more informative solutions. 

\section{A realistic setup : teacher-student regression}

Our work has shown the emergence of a crossover time in a class of optimization problems, before which one should keep the learning rate constant and after which it becomes useful to decay the learning rate. 

To investigate whether these findings hold in more realistic setups, we turn to a teacher-student regression problem involving two-layer neural networks. Our setup is similar to the online setting of~\cite{saad1995line}, later studied by ~\cite{goldt2020dynamics}, except that we consider a finite dataset.

More precisely, consider learning a high-dimensional "teacher" function $T:\mathbb R^N \rightarrow \mathbb R$ given by a two-layer network with a "student" two-layer network:
\begin{align}
    T(\spin) = \sum_{m=1}^M v^*_m g\left(\frac{w^*_m \cdot \spin}{\sqrt{N}}\right) \quad\quad\quad 
    S(\spin) = \sum_{k=1}^K v_k g \left(\frac{w_m \cdot \spin}{\sqrt{N}}\right)
\end{align}

The learning task consists in minimizing the mean-squared error over a set of $P$ observations:
\begin{align}
    \loss = \frac{1}{2P} \sum_{\mu=1}^P \left(S(\spin_\mu) - T(\spin_\mu)\right)^2
\end{align}

To be able to observe convergence rates, we need a situation in which we know the ground state, and the model can find the ground state. For this, we need the student to have sufficient capacity to fit the teacher, i.e. $K\geq M$, and we need a small enough dataset for the student to be able to interpolate the data, i.e. $P<KN$. To add noise in the problem, we add a random corruption to the observations at each step, as in Langevin dynamics. 

Similarly to Sec.~\ref{sec:crossover}, we investigate the existence of a crossover time in the dynamics in Fig.~\ref{fig:crossover-nn}. To do so, we keep the learning rate constant, then decay it at various times. We see that if we start decaying too early, the decay slows down the descent; ideally, the decay must start when the training loss starts to saturate due to the temperature, exactly as seen in the Sherrington-Kirkpatrick model.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.5\linewidth}
    \includegraphics[width=\linewidth]{figs/energy_nn_H50.pdf}
    %\caption{50 hidden nodes}
    \end{subfigure}
    \caption{How different learning rate schedules affect the energy as function of time. We set $N=50$, $P=100$, $T=0.1$, $\lr_0=0.1$.}
    \label{fig:crossover-nn}
\end{figure}

